Latent Space Interpretation for Stylistic Analysis and Explainable Authorship Attribution

Recent state-of-the-art authorship attribution methods learn authorship representations of texts in a latent, non-interpretable space, hindering their usability in real-world applications. Our work proposes a novel approach to interpreting these learned embeddings by identifying representative points in the latent space and utilizing LLMs to generate informative natural language descriptions of the writing style of each point. We evaluate the alignment of our interpretable space with the latent one and find that it achieves the best prediction agreement compared to other baselines. Additionally, we conduct a human evaluation to assess the quality of these style descriptions, validating their utility as explanations for the latent space. Finally, we investigate whether human performance on the challenging AA task improves when aided by our system's explanations, finding an average improvement of around +20% in accuracy.

==> sections/analysis.tex <==
\section{Analysis}\label{sec:analysis}

\begin{figure*}[t]
    \centering
    \begin{minipage}[b]{0.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/style_consistency.pdf} 
        \caption{Evolution of stability $S_t$ across time steps $t$, with shaded error bands representing the standard deviation.}
        \label{fig:style_consistency}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.6\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/style_topic_correlation.pdf} 
        \caption{Correlation statistics between embeddings, styles, and topics. For metrics, cosine similarity is used for embeddings and symmetric KL divergence is used for style and topic representations.}
        \label{fig:style_topic_correlation}
    \end{minipage}
\end{figure*}

\paragraph{Are Style Assignments by LLMs Consistent?}
To ensure the generated style descriptions are reliable and not spuriously generated, we validate the consistency of style descriptions produced by LLMs across different query instances. Specifically, we prompt \llama with documents from the same author multiple times and evaluate the stability of the resulting style distribution. At each time step $t \in \mathbb{N}$, we compute the style distribution $v^d_t \in \Delta^k$ and take the unweighted average of all previously generated distributions as $\bar{v}^d_t = \frac{1}{t}\sum_{i=1}^t v^d_i$. Denoting stability at step $t$ as $S_t$, we evaluate $S_t$ for $t \leq 25$ as the symmetrized Kullback-Leibler (KL) divergence between the averaged style distributions of step-adjacent instances:
\begin{equation*}
    S_t = \frac{1}{2}\left(D_{\text{KL}}(\bar{v}^d_{t} \parallel \bar{v}^d_{t-1}) + D_{\text{KL}}(\bar{v}^d_{t-1} \parallel \bar{v}^d_{t}) \right).
\end{equation*}

To mitigate potential consistency illusions from using identical prompt instructions, we manually generate 20 paraphrased variants of the original instruction and sample an instruction uniformly at random for each query. Given the known variability of LLMs when processing semantically identical inputs \cite{jiang-etal-2020-know, elazar-etal-2021-measuring, zhou2022promptconsistencyzeroshottask}, observing convergence in style assignments across these varied prompts suggests that LLMs maintain consistency in generating style descriptions. Detailed prompt examples are provided in Appendix \ref{app:style_consistency}.

Results are shown in Figure~\ref{fig:style_consistency}. Observe that stability converges to the minimum value after 20 rounds, demonstrating that LLM-generated styles are consistent across multiple prompting instances. These results suggest that author-level style assignments are both representative and consistent. \bscom[]{}{MA: I see now how this could be used against our approach. According to the graph, we should have run our code up to 20 times and computed the final style distribution of each cluster as the average of all the runs. We might want to move the whole thing into the appendix and only slightly mention this, probably in the limitation.}

%\paragraph{Style/topic entanglement.}
\paragraph{What do Authorship Attribution Models Represent?}
Previous studies \citep{rivera-soto-etal-2021-learning, wang-etal-2023-authorship} have observed the \bscom{correlation between the learned latent representations of authorship attribution models and document topics}{the learned representation of authorship attribution models doesn't only capture writing styles of texts but also their topics}. Therefore, we investigate whether the document's latent representations captured by authorship attribution models correlate with their style or topic representation. Concretely, we obtain three representations for each author: style, topic, and authorship attribution latent representation. We obtain the authorship attribution latent representation by averaging the author's document embeddings generated by the authorship attribution model. We run our method described in Section~\ref{sec:latent_space_interpretation} to obtain style representations. As for topic representations, we use BERTopic \citep{grootendorst2022bertopic} to compute the topic representation of each document and average them to get the final topic representation of the author. We then compute pairwise dissimilarities between authors using cosine similarity for latent representations and symmetric KL divergence for style and topic representations. To obtain correlation scores, we use distance correlation \citep{Sz_kely_2007},\bscom[Is there value of showing the two different correlation measures? if no then we can just show only one that captures our message that we want to convey]{}{ which seeks to capture linear and non-linear relationships, and Pearson correlation, which captures linear relationships.}

Results are shown in Figure~\ref{fig:style_topic_correlation}. \bscom[]{Observe that style consistently shows a higher correlation with the embeddings compared to topics across both correlation results}{Despite the relatively high correlation between authors' dissimilarity in the latent space and the dissimilarity of their topic, we also observe that the correlation is higher when we compare this dissimilarity in the latent and style representation. This indicates that authors who are similar in the authorship attribution latent space have, to some degree, similar writing styles.}.

==> tables/alignment_performance.tex <==
\begin{table*}[t!]
    \small
    \setlength{\tabcolsep}{3pt}    
    \centering
    \begin{tabular}{llllrrr}
        \toprule
        & & \textbf{Measure 1} & \textbf{Measure 2} & \textbf{Distance Correlation} & \textbf{Pearson Rank} & \textbf{Spearman Rank} \\ 
        \midrule
        \multirow{4}{*}{\textbf{Embeddings}} & \multirow{4}{*}{$\leftrightarrow$ \textbf{Styles}} & Euclidean & KL Div.\ & 0.459 & 0.241 & 0.284 \\
        & & Euclidean & KL Div.\ (Sym.) & 0.484 & 0.279 & 0.325 \\
        & & Cosine & KL Div.\ & 0.445 & 0.184 & 0.235 \\
        & & Cosine & KL Div.\ (Sym.) & 0.469 & 0.213 & 0.261 \\
        \midrule
        \multirow{4}{*}{\textbf{Embeddings}} & \multirow{4}{*}{$\leftrightarrow$ \textbf{Topics}} & Euclidean & KL Div.\ & 0.401 & 0.148 & 0.360 \\
        & & Euclidean & KL Div.\ (Sym.) & 0.429 & 0.174 & 0.346 \\
        & & Cosine & KL Div.\ & 0.411 & 0.149 & 0.342 \\
        & & Cosine & KL Div.\ (Sym.) & 0.441 & 0.172 & 0.340 \\
        \midrule
        \multirow{4}{*}{\textbf{Styles}} & \multirow{4}{*}{$\leftrightarrow$ \textbf{Topics}} & KL Div.\ & KL Div.\ & 0.437 & 0.234 & 0.296 \\
        & & KL Div.\ & KL Div.\ (Sym.) & 0.373 & 0.188 & 0.249 \\
        & & KL Div.\ (Sym.) & KL Div.\ & 0.386 & 0.198 & 0.291 \\
        & & KL Div.\ (Sym.) & KL Div.\ (Sym.) & 0.387 & 0.225 & 0.301 \\
        \bottomrule
    \end{tabular}
    \caption{\label{tab:alignment_performance} Distance Correlation Scores between Styles, Embeddings, and Topics. \edward{Just a placeholder for now, will drastically edit soon}}
\end{table*}

==> tables/user_study_one_annotator_agreement.tex <==
\begin{table}[t!]
    \small
    \setlength{\tabcolsep}{3pt}    
    \centering
    \begin{tabular}{lrrrrr}
        \toprule
        & \multicolumn{4}{c}{\bf  Kendall's $\tau$} &  \bf Kendall's w \\
        & \bf ann1\&2 & \bf ann1\&3 & \bf ann2\&3 & \bf AVG.\\
        \midrule
        \bf G1 & 0.40 & 0.03 & 0.10 & 0.18 & 0.48 \\
        \bf G2 & -0.20 & 0.13 & -0.07 & -0.04 & 0.29 \\
        \bottomrule
    \end{tabular}
    \caption{\label{tab:user_study_1_aa} Annotators agreement of both Group 1 (G1) and Group 2 (G2) measured using Kendall's $\tau$ and Kendall's $w$. }
\end{table}

